Incentivising Exploration and Recommendations for Contextual Bandits with Payments

We propose a contextual bandit based model to capture the learning and social welfare goals of a web platform in the presence of myopic users. By using payments to incentivize these agents to explore different items/recommendations, we show how the platform can learn the inherent attributes of items and achieve a sublinear regret while maximizing cumulative social welfare. We also calculate theoretical bounds on the cumulative costs of incentivization to the platform. Unlike previous works in this domain, we consider contexts to be completely adversarial, and the behavior of the adversary is unknown to the platform. Our approach can improve various engagement metrics of users on e-commerce stores, recommendation engines and matching platforms.

==> analysis.tex <==

\section{Guarantees on Total Payments \& Regret}\label{sec:analysis_results}

We provide expected regret and expected payment guarantees for a few of the approaches outlined in Section~\ref{sec:algorithm}, where the expectation is with respect to the internal randomness of the approach unless otherwise stated. 

\begin{comment}

To start with, we list out a collection of assumptions, some of which will be needed for the results to hold (different approaches require different assumptions).
\todo{To discuss: There are two different types of co-variate diversity and margin assumptions. Both requires some description of model, e.g. for noisy contexts, we should explain noise generation. Should all that be described here?}\\

\begin{enumerate}
    \item[A1] a
    \item[A2] a
\end{enumerate}

\end{comment}

\subsection{The Unrestricted Budget Scenario}

\textbf{Approach 1: Adapting Generic Contextual Bandit Algorithms}

While the sublinear regret guarantees for \PaymentProfile~ immediately follow from the corresponding contextual bandit results, the expected payments incurred can be as large as $O(T)$.


\textbf{Approach 2: Payments as a Source of User Heterogeneity}

\textbf{Approach 3: Adapting the Chaining Approach of Kannan et al. ~\cite{kannan2017fairness}}
\begin{comment}
In \UnrestrictedBudget, the confidence width is central to the notion of chained set. The following lemma gives a high probability bound on the size of confidence width at any given round $t$.
\begin{lemma}\label{lem:confidence_width}
[Theorem~3 in~\cite{joseph2016rawlsian} \& Theorem~2 in~\cite{abbasi2011improved}] In \UnrestrictedBudget, for $\est^t_i= (\Theta(S_{i,t-1})^T_i\Theta(S_{i,t-1})+\lambda I)^{-1}\Theta(S_{i,t-1})^T Y(S_{i,t-1})$,\todo{[Change notation! what is the pobablity over/source of randomness here?]} where $\Theta(S_{i,t-1})$ and $Y(S_{i,t-1})$ are design matrices and observations till $t-1$ with $\vert \vert X \vert \vert_2 \leq 1$ , for all $ t\geq 1$ and $\delta >0$, then the following holds with $1-\delta$ probability (the source of randomness here is noise in the rewards):
\begin{equation}
    w^t_i = \theta_t.\vert \mu_i - \est^{t-1}_i \vert \leq \vert \vert \theta_t \vert \vert_{(X^t_iX_i+\lambda I)^{-1}} \left(m\sqrt{d\log\left(\frac{1+t/\lambda}{\delta}\right)}+\sqrt{\lambda}\right)
\end{equation}
\end{lemma}

\end{comment}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The Restricted Budget Scenario}


%State the result of Colt/Frazier

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The No Budget Scenario}
\todo{We can qualitatively highlight the results of bastani for K=2 and COlT paper, we are already beyond 8 pages.}
%State the result of Bastani and Kannan18









